IPv6 Hitlists at Scale: Be Careful What You Wish For

Today's network measurements rely heavily on Internet-wide scanning, employing tools like ZMap that are capable of quickly iterating over the entire IPv4 address space. Unfortunately, IPv6's vast address space poses an existential threat for Internet-wide scans and traditional network measurement techniques. To address this reality, efforts are underway to develop ``hitlists'' of known-active IPv6 addresses to reduce the search space for would-be scanners. As a result, there is an inexorable push for constructing as large and complete a hitlist as possible. This paper asks: what are the potential benefits and harms when IPv6 hitlists grow larger? To answer this question, we obtain the largest IPv6 active-address list to date: 7.9 billion addresses, 898 times larger than the current state-of-the-art hitlist. Although our list is not comprehensive, it is a significant step forward and provides a glimpse into the type of analyses possible with more complete hitlists. We compare our dataset to prior IPv6 hitlists and show both benefits and dangers. The benefits include improved insight into client devices (prior datasets consist primarily of routers), outage detection, IPv6 roll-out, previously unknown aliased networks, and address assignment strategies. The dangers, unfortunately, are severe: we expose widespread instances of addresses that permit user tracking and device geolocation, and a dearth of firewalls in home networks. We discuss ethics and security guidelines to ensure a safe path towards more complete hitlists.

==> Makefile <==
TARGET := submission
BIB := refs.bib

TEX_ALL := $(shell search=$(TARGET).tex; all=; \
				while [ -n "$$search" ] ; do \
					all="$$all $$search"; \
					search=`grep -E "^[^%]*input" $$search | \
						sed -En 's/.*input[^\{]*\{(.+)\}/\1.tex/p'`; \
				done; \
				echo "$$all")

FIGURES := $(shell for t in $(TEX_ALL); do \
				cat $$t | \
				grep -E '^[^%]*\\includegraphics' | \
				sed -En 's/.*includegraphics(\[.+\])?\{([^\{]*)\}.*/\2/p' | \
				grep -E -v '\.pdf$$'; \
				done)

# Package acronym Warning: Acronym `CDN'
all: $(TARGET).pdf
	@mm=`grep "Warning: Citation" $(TARGET).log | sort | uniq | wc -l | awk '{print $$1;}'`; \
	 nn=`grep "Warning: Reference" $(TARGET).log | sort | uniq | wc -l | awk '{print $$1;}'`;  \
	 oo=`grep "Warning: Label " $(TARGET).log | sort | uniq | wc -l | awk '{print $$1;}'`;  \
	 pp=`grep "Package acronym Warning: Acronym " $(TARGET).log | sort | uniq | wc -l | awk '{print $$1;}'`;  \
	 if [ $$mm -eq 0 -a $$nn -eq 0 -a $$oo -eq 0 -a $$pp -eq 0 ]; then \
	 	echo "\033[0;34mZero missing citations and references! 👏🎉\033[0m"; \
	 else \
		 echo "\033[1;33m################################"; \
		 if [ $$mm -gt 0 ]; then \
			 echo "$$mm missing citation(s):"; \
			 grep "Warning: Citation" $(TARGET).log | awk '{print "\033[0;31m   ", $$5;}' | sed "s/[\`']//g" | sort | uniq; \
		 fi; \
		 if [ $$nn -gt 0 ]; then \
			 echo "\033[1;33m$$nn missing reference(s):"; \
			 grep "Warning: Reference" $(TARGET).log | awk '{print "\033[0;31m   ", $$4;}' | sed "s/[\`']//g" | sort | uniq; \
		 fi; \
		 if [ $$oo -gt 0 ]; then \
			 echo "\033[1;33m$$oo multiply defined label(s):"; \
			 grep "Warning: Label" $(TARGET).log | awk '{print "\033[0;31m   ", $$4;}' | sed "s/[\`']//g" | sort | uniq; \
		 fi; \
		 if [ $$pp -gt 0 ]; then \
			 echo "\033[1;33m$$pp undefined acronym(s):"; \
			 grep "Package acronym Warning: Acronym" $(TARGET).log | awk '{print "\033[0;31m   ", $$5;}' | sed "s/[\`']//g" | sort | uniq; \
		 fi; \
		 echo "\033[1;33m################################\033[0m"; \
	 fi

$(TARGET).pdf: $(TEX_ALL) $(BIB)
	pdflatex $(TARGET).tex
	bibtex $(TARGET)
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex

view:: $(TARGET).pdf
	open $(TARGET).pdf

see:: $(TARGET).dvi
	xdvi $(TARGET)

spell::
	ispell *.tex

clean::
	rm -fv *.dvi *.aux *.log *~ *.bbl *.blg *.toc *.out *.ps *.pdf *.ent parsetab.py

fresh::
	rm -fv *.dvi *.aux *.log *~ *.bbl *.blg *.toc *.ps *.pdf

distclean:: clean
	rm $(TARGET).ps

.PHONY: clean all view see spell fresh distclean nobib

